LS-VO: Learning Dense Optical Subspace for Robust Visual Odometry Estimation

This work proposes a novel deep network architecture to solve the camera Ego-Motion estimation problem. A motion estimation network generally learns features similar to Optical Flow (OF) fields starting from sequences of images. This OF can be described by a lower dimensional latent space. Previous research has shown how to find linear approximations of this space. We propose to use an Auto-Encoder network to find a non-linear representation of the OF manifold. In addition, we propose to learn the latent space jointly with the estimation task, so that the learned OF features become a more robust description of the OF input. We call this novel architecture LS-VO. The experiments show that LS-VO achieves a considerable increase in performances in respect to baselines, while the number of parameters of the estimation network only slightly increases.

==> settings/def_macros.tex <==
\newcommand\inputfile[1]{%
  \InputIfFileExists{#1}{}{\typeout{No file #1.}}%
}
\newcommand{\todo}[1]{\noindent\textbf{\textcolor{red}{[TODO: #1]}}}


\makeatletter
\DeclareRobustCommand\icgonedot{\futurelet\@let@token\@icgonedot}
\newcommand\@icgonedot{\ifx\@let@token.\else.\null\fi\xspace}
\newcommand\eg{\textit{e.g}\icgonedot}
\newcommand\Eg{\textit{E.g}\icgonedot}
\newcommand\ie{\textit{i.e}\icgonedot} 
\newcommand\Ie{\textit{I.e}\icgonedot}
\newcommand\ia{\textit{i.a}\icgonedot}
\newcommand\Ia{\textit{I.a}\icgonedot}
\newcommand\cf{\textit{cf}\icgonedot} 
\newcommand\Cf{\textit{C.f}\icgonedot}
\newcommand\etc{\textit{etc}\icgonedot}
\newcommand\vs{\textit{vs}\icgonedot}
\newcommand\wrt{w.r.t\icgonedot}
\newcommand\aka{a.k.a\icgonedot}
\newcommand\dof{d.o.f\icgonedot}
\newcommand\etal{et al\icgonedot}
\newcommand\OFC{\textrm{OFC}\xspace}

%Added by thomas
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\xb}{\mbf{x}}
\newcommand{\Xb}{\mbf{X}}
\newcommand{\yb}{\mbf{y}}
\newcommand{\zb}{\mbf{z}}
\newcommand{\hb}{\mbf{h}}
\newcommand{\ub}{\mbf{u}}
\newcommand{\Wk}[1]{\mbf{W}_k^{#1}}
\newcommand{\xbp}{\mbf{x^\prime}}
\newcommand{\txb}{\mbf{\tilde{x}}}
\newcommand{\txbp}{\mbf{\tilde{x}^\prime}}
\newcommand{\T}[1]{#1^\mathsf{T}}
\newcommand{\RR}{I\!\!R}
\newcommand{\Mbb}{\mathbb{M}}
\newcommand{\Obb}{\mathbb{O}}
\newcommand{\Zbb}{\mathbb{Z}}
\newcommand{\Ybb}{\mathbb{Y}}
\newcommand{\Rbb}{\mathbb{R}}


\makeatother

